Single-Pass Contrastive Learning Can Work for Both Homophilic and Heterophilic Graph

Existing graph contrastive learning (GCL) techniques typically require two forward passes for a single instance to construct the contrastive loss, which is effective for capturing the low-frequency signals of node features. Such a dual-pass design has shown empirical success on homophilic graphs, but its effectiveness on heterophilic graphs, where directly connected nodes typically have different labels, is unknown. In addition, existing GCL approaches fail to provide strong performance guarantees. Coupled with the unpredictability of GCL approaches on heterophilic graphs, their applicability in real-world contexts is limited. Then, a natural question arises: Can we design a GCL method that works for both homophilic and heterophilic graphs with a performance guarantee? To answer this question, we theoretically study the concentration property of features obtained by neighborhood aggregation on homophilic and heterophilic graphs, introduce the single-pass augmentation-free graph contrastive learning loss based on the property, and provide performance guarantees for the minimizer of the loss on downstream tasks. As a direct consequence of our analysis, we implement the Single-Pass Graph Contrastive Learning method (SP-GCL). Empirically, on 14 benchmark datasets with varying degrees of homophily, the features learned by the SP-GCL can match or outperform existing strong baselines with significantly less computational overhead, which demonstrates the usefulness of our findings in real-world cases.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sec-analysis.tex <==
% \section{Revisiting Graph Augmentations}
\section{An Experimental Investigation}
\label{sec:aug_study}
Graph Contrastive Learning (GCL) aims to learn representations that are invariant to different augmentations. However, it is rarely studied what information is preserved or perturbed across augmented graph views. In this section, we attempt to identify such information by examining the effect of graph augmentation techniques on graph geometric structure and node attributes from the spectral perspective.

\subsection{Representative Augmentation Techniques}
According to Table~\ref{tab:graph_aug_summary}, the most commonly used four graph augmentation techniques for GCL are: attribute masking, edge adding, edge dropping~\cite{you2020graph} and graph diffusion~\cite{you2020graph}.
\begin{itemize}
  \item Attribute Masking: randomly masks a fraction of features for all the nodes.
  \item Edge Adding/Dropping: randomly adds/drops a fraction of edges from the original graph.
  \item Graph Diffusion: the Personalized PageRank (PPR) based graph diffusion is defined as, $\alpha\left(\mathbf{I}-(1-\alpha) \mathbf{A}_{sym}\right)^{-1}$, where $\alpha$ is the diffusion factor.
\end{itemize}
\subsection{Effect of Augmentations on Geometric Structure}
\begin{wrapfigure}{r}{0.4\textwidth}
\vspace{-45pt}
  \begin{center}
    \includegraphics[width=1.0\textwidth]{images/ER0.2_FM0.2_new.pdf}
  \end{center}
  \vspace{-10pt}
  \caption{{Frobenius distance between the decomposed symmetric normalized Laplacian matrices of the original graph and the augmented graph with 20\% edge dropping.} The experiment is independent conducted 10 times and the average value is reported.}
  \label{fig:er_fm_observation}
\vspace{-10pt}
\end{wrapfigure}
First, we investigate the effect of different augmentations, e.g., edge adding, edge dropping and graph diffusion, on adjacency matrix.
As we introduced in Section~\ref{subsec:laplacian_concept}, the graph Laplacians are widely used in GNNs, therefore we measure the difference of Laplacians caused by graph augmentations in different frequency bands.
The $m$-th component symmetric normalized Laplacian is defined as ${\mathbf{L}}^{m}_{sym}$. Correspondingly, we denote the decomposed $m$-th symmetric normalized Laplacian for the augmented graph as ${\widetilde{\mathbf{L}}}_{sym}^{m}$. 
To measure the impact of graph augmentations for different frequency components, we employ the Frobenius norm as the metric to measure the distance, $\|{\mathbf{L}}^{m}_{sym} - {\widetilde{\mathbf{L}}}^{m}_{sym}\|_F$. 
% \qi{any reference between this term and frequency changes?}
%, to measure the effect of edge adding, edge dropping and graph diffusion on different frequency components. 
The results of edge dropping on two homophilic graphs, e.g., Cora and CiteSeer~\cite{sen2008collective, namata2012query}, and two heterophilic graphs, e.g., Chameleon and Squirrel~\cite{rozemberczki2021twitch}, are summarized in Figure~\ref{fig:er_fm_observation} and the results of other graph augmentation techniques are in Appendix~\ref{apd:aug_study}. We observed that graph augmentations have less impact on low-frequency components and more impact on middle and high-frequency components. 
Our conclusion is aligned with the previous works~\cite{entezari2020all, chang2021not} in the graph adversarial attack domain, in which they find that, for the graph structure modification, perturbations on the low-frequency components are smaller than that in the middle or high-frequency ones.
% \begin{figure}[h]
% \vspace{-5pt}
% \centering
% \includegraphics[width=0.43\textwidth]{images/ER0.2_FM0.2_new.eps}
% \vspace{-5pt}
% \caption{{Frobenius distance between the decomposed symmetric normalized Laplacian matrices of the original graph and the augmented graph with 20\% edge dropping.} 
% The experiment is independent conducted 10 times and the average value is reported.}
% \label{fig:er_fm_observation}
% \vspace{-5pt}
% \end{figure}
\subsection{Effect of Augmentations on Features}
\vspace{-5pt}
\begin{wraptable}{r}{6cm}
\vspace{-20pt}
\caption{Distance between original node features and augmented node features with 30\% attribute dropping. We set $R=0.8\times F$.}
\label{tab:feat_freq_analysis}
\begin{tabular}{ccc}\\
\toprule
 & F-Low & F-High \\\hline
Cora & 0 & 7.949 \\  \hline
CiteSeer & 0 & 5.609 \\  \hline
Chameleon & 0 & 12.566 \\  \hline
Squirrel & 0 & 15.836 \\  
\bottomrule
\end{tabular}
\end{wraptable} 
To further study the effect of the commonly used graph augmentation method, attribute masking, on node attribute from spectral view. We denote the Fourier transform and inverse Fourier transform as $\mathcal{F}(\cdot)$ and $\mathcal{F}^{-1}(\cdot)$.
We use $\mathbf{H}^\mathcal{F}$ to denote the transformed node features. Therefore, we have $\mathbf{H}^{\mathcal{F}}=\mathcal{F}(\mathbf{X})$ and $\mathbf{X}=\mathcal{F}^{-1}(\mathbf{H}^{\mathcal{F}})$.
We decompose the node attribute $\mathbf{X}=\left\{\mathbf{X}^{l}, \mathbf{X}^{h}\right\}$, where $\mathbf{X}^{l}$ and $\mathbf{X}^{h}$ denote the low-frequency and high-frequency components of $\mathbf{X}$ respectively. We have the following four equations:
$$
\begin{array}{rlr}
\mathbf{H}^{\mathcal{F}}=\mathcal{F}(\mathbf{X}), & \mathbf{H}^{l}, \mathbf{H}^{h}=t(\mathbf{H}^{\mathcal{F}}; R), \\
\mathbf{X}^{l}={\mathcal{F}}^{-1}\left(\mathbf{H}^{l}\right), & \mathbf{X}^{h}=\mathcal{F}^{-1}\left(\mathbf{H}^{\mathcal{F}}\right),
\end{array}
$$
where $t(\cdot ; R)$ denotes a thresholding function that separates the low and high frequency components from $\mathbf{H}^f$ according to a hyperparameter, $m$. Because the column of $\mathbf{H}^{\mathcal{F}}$ in the left is corresponding to the low frequency component, we define $t(\cdot ; m)$ as:
\begin{equation}
\begin{aligned}
&\mathbf{H}^{l}_{ij}= \begin{cases}\mathbf{H}^{\mathcal{F}}_{ij}, & \text { if } j \leq R \\
0, & \text { otherwise }\end{cases}, 
&\mathbf{H}^{h}_{ij}= \begin{cases}0, & \text { if } j \leq R \\
\mathbf{H}^{\mathcal{F}}_{ij}, & \text { otherwise }\end{cases}.
\end{aligned}
\end{equation}
Further, we denote the node attribute with attribute masking as $\widetilde{\mathbf{X}}$ and its corresponding low and high frequency components as $\widetilde{\mathbf{X}}^l$, $\widetilde{\mathbf{X}}^h$.
% Setting $m=\ceil{0.8*F}$, 
We investigate the influence of attribute masking on node features by computing the Frobenius distance of matrix, and denote $\|{\mathbf{X}}^l - \widetilde{\mathbf{X}}^l \|_F$ as F-norm-low
and  $\|{\mathbf{X}}^h - \widetilde{\mathbf{X}}^h \|_F$ as F-norm-high.
The results on four datasets are summrized in Table~\ref{tab:feat_freq_analysis}. We surprisingly find that the attribute masking will always affect the high frequency component.
% \begin{table}[h]
% \label{tab:feat_freq_analysis}
% \caption{Distance between original node features and augmented node features with 30\% attribute dropping. We set $R=0.8\times F$.} 
% \centering
% \begin{tabular}{l|c|c}
% \toprule
% \multicolumn{1}{r|}{} & \multicolumn{1}{r|}{F-Norm-Low} & \multicolumn{1}{r}{F-Norm-High} \\ \hline
% Cora                   & 0                               & 7.949                           \\ \hline
% CiteSeer               & 0                               & 5.609                           \\ \hline
% Chameleon              & 0                               & 12.566                          \\ \hline
% Squirrel               & 0                               & 15.836                          \\ 
% \bottomrule
% \end{tabular}
% \end{table}
\subsection{Concluding Remarks}
As demonstrated by previous works~\cite{bo2021beyond, li2021beyond},  for heterophilic graphs, the information carried by high-frequency components is more effective for downstream classification performance.
However, as we analyzed, the middle- and high-frequency information are perturbed by commonly used graph augmentation techniques. With the information maximization objective, only the invariant information (low-frequency) is encouraged to be captured by the learned embedding~\cite{you2020graph}.
Although existing graph augmentation algorithms promote the success of GCL on traditional (homophilic) benchmarks, they result in sub-optimal representations when the high-frequency information is crucial (heterophilic graphs).

% In all, the four graph augmentation techniques for node-level representation learning tend to preserve the low-frequency information and perturb the high-frequency information.
% Therefore, the self-supervision signal constructed based on those techniques facilitate the learning of low-frequency, which is critical for the representation learning on homophilic graph. However, for the heterophilic graph, in which the low-frequency information is insufficient to support the inference, the augmentation-based GCL methods could hardly capture the high-frequency information and therefore result in sub-optimal representations.

% By enforcing the model to learn representations invariant to the perturbations through maximizing the agreement between a graph and its augmentation, learned representations are invariant to high-frequency information while retaining low-frequency information.
% As demonstrated in~\cite{balcilar2020analyzing}, the low-frequency information is critical for homophilic graph. However, for the heterophilic graph, the low-frequency information is insufficient to support the inference in such networks. Under the circumstances, the high-frequency information, capturing the difference between nodes, maybe more suitable~\cite{zhu2020beyond, luan2021heterophily}.
% This nature of the heterophilic graph hinders the application of the previous GCL algorithms.

